What's in your hands? 3D Reconstruction of Generic Objects in Hands

Our work aims to reconstruct hand-held objects given a single RGB image. In contrast to prior works that typically assume known 3D templates and reduce the problem to 3D pose estimation, our work reconstructs generic hand-held object without knowing their 3D templates. Our key insight is that hand articulation is highly predictive of the object shape, and we propose an approach that conditionally reconstructs the object based on the articulation and the visual input. Given an image depicting a hand-held object, we first use off-the-shelf systems to estimate the underlying hand pose and then infer the object shape in a normalized hand-centric coordinate frame. We parameterized the object by signed distance which are inferred by an implicit network which leverages the information from both visual feature and articulation-aware coordinates to process a query point. We perform experiments across three datasets and show that our method consistently outperforms baselines and is able to reconstruct a diverse set of objects. We analyze the benefits and robustness of explicit articulation conditioning and also show that this allows the hand pose estimation to further improve in test-time optimization.

==> 1_intro.tex <==
\section{Introduction}

% \todo{ensure we are using correct sty file and format}.
% \todo{1. teaser, qualitative results. }

% We aim to perceive HOI for generic object. some example. bc human do, useful for ego centric, robotcis, etc. 

% Community has achieved Recent years hand/object recon has pushed for in-the-wild

% hoi are challenging, bc self occlusion...


% Given an image depicting a hand holding a pen, humans can perceive hand fingers pinching together  which a long stick pass through. We understand that the pen  

Humans  interact with their surrounding world with their hand. Not only do we understand  interaction as abstract concepts such as touching screen,  squeezing balls, holding pens, \etc, we also perceive their underlying 3D shape. Holding a pen means a stick lying on purlicue and  gripped by thumb, index and middle fingers; holding a bowl is placing it on top of an upfacing palm. We aim to build a recognition system that can perceive and reason about the geometric information 
hand-object interactions (HOI) for generic objects.

% \todo{change to another motivating example for reconstruction? --> start with impact?  Humans interact with the surrounding world with their hands with strong priors about the  object geometry. Cups and plates are grasped differently as ones are cylinder-like and the others are flat, while electric drills and tennis rackets are grasped similarly because their handles share similar local shapes. This geometry reasoning about local shape can generalize to diverse set of objects in our daily life such as  pens, markers, mugs, spray bottles, \etc. We are able to infer hand-object interaction in 3D even if we have not encountered such specific object. We aim to build a recognition system that can perceive and reason about the geometric information 
% hand-object interactions (HOI) for generic objects. }

Understanding HOI  for generic objects with 3D information has the potential to help understand ego-centric daily videos at large scale, of which a great portion captures hand manipulating objects \cite{ego4d, epic}. It could also help to advance dexterous hand manipulation where robots learn to manipulate from human demonstration \cite{dexmv, kristen}.

\todo{maybe cut it to 3 sentences?  In recent years, the community has advanced in inferring 3D shape for hand or object alone, especially in terms of generalizing them to unseen in-the-wild settings. 
Hand poses can be recovered in the form of 2D keypoints \cite{}, 3D joint location \cite{}, or even full 3D meshes \cite{boulk, frankmocap} via either fitting templates or direct regression. The hand prediction from off-the-shelf system is generally robust to occlusion and diverse appearance for an arbitrary image. Meanwhile, recent works have pursued scaling object reconstruction from estimating 6D pose for one specific known object to more generic objects, such as various instances within one category  \cite{shelf,umr, cmr}, or even pursuing a joint model for cross-category reconstruction \cite{mesh}. Other works also study expressive and flexible 3D representation \cite{deepsdf, cmf}, to represent objects exhibiting large shape variance \etc. We are able to lift an image of isolated objects to the underlying coarse 3D shape for  a wide range of common objects. However, they typically assume little occlusion which does not hold for HOI.
}
% Some other works \cite{occpancy, sdf, imnet} have proposed to represent 3D shape as level-set of intrinsic implicit function approximated by  neural network. This allows for more flexible and accurate reconstruction in high resolution. \todo{improve flow}


While we have made impressive parrallel progress in hand / object reconstruction in the wild, HOI reconstruction in the wild is highly challenging and ill-posed due to lack of data, mutual and self-occlusion. Prior works \cite{HO3d} typically focus on reconstructing a handful of known object under lab environment. There have been recent efforts to go beyond lab setting to increase appearance diversity such as mining hard examples from videos, introducing large-scale dataset\cite{100doh, ego4d}, leveraging 2D observation to fit template \cite{zhe, homan}, etc. However, fewer works study to relax the requirement of known objects. Most of prior HOI reconstruction method still work on known objects by assuming access to 3D templates of the objects and reduce reconstruction to a 6D pose estimation problem. 
We argue that knowing the 3D template of the object as a priori during inference is a strong assumption and prevents their systems from reconstructing unknown objects.
Furthermore, they struggle to handle various object shape in the wild as these templates are rigid and instance specific.  In contrast, our work studies hand-object reconstruction without object templates and instead focuses on reconstructing HOI for novel objects from images.  

% \todo{instance specific template, know object before hand in test time, reduce to pose estimation. }
% However, HOI reconstruction in the wild is highly challenging and ill-posed due to mutual and self occlusion.  Most prior works assume access to the 3D templates of the objects. These templates are rigid and instance specific. By knowing the template as a priori, the reconstruction problem is reduced to a 6D pose estimation problem. 
% The videos are captured in control lab settings with limited appearance diversity. These limitations prevent previous methods from generalizing to novel shapes that are not in the template repository, or from scaling up recognition to in-the-wild data. 

% Although there have been great progresses on HOI reconstruction \cite{shaowei, yana, rhoi}, they typically work on a small set of objects like a subset of YCB objects. 

Our key observation is that hand articulation is driven by the local geometry of the object thus hand articulation provides strong cues for the object in interaction. Fingers curled like fist indicate thin handles in between while open palms are likely to interact with flat surfaces. 
% exploit
Instead of treating the hand occlusion as noise to marginalize over, we explicitly consider hand pose as informative cues for the object it interacts with. 
We operationalize this idea by conditionally predicting the object shape based on hand articulation and  the input image. Instead of estimating both hand pose and object shape jointly, we leverage advances in hand pose reconstruction to estimate hand pose first. Given the inferred articulated hand along with the input image, our approach then reconstruct the object in a normalized hand-centric coordinate frame.
We formulate the object shape as a point-wise implicit function that maps a point to distance to the object surface conditioned on pixel-aligned visual feature and articulation-aware coordinates. 

We evaluate our method across three datasets including synthetic and real-world benchmarks and compare ours with prior explicit and implicit HOI reconstruction methods that infer shape of unknown objects independent of hand pose. Our articulation-conditioned object shape prediction consistently outperform baselines by a large margin and can reconstruct various objects in wide range of shape. We also analyze how our model benefits from articulation-aware coordinates. Lastly, we show that the initial hand pose estimation could be further improved by encouraging interaction between the predicted hand and object.   

% sdf
% At inference time, given an image, we first apply off-the-shelf hand-only reconstructors and then use the learned prior to infer the shape within hands. We show that the articulation-conditioned model is able to generalize better to novel objects for data in the wild. 


==> fig/coord.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/coord.png}
    \caption{}
    \label{fig:coord}
\end{figure}

==> fig/fk.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/fk.png}
    \caption{This is so ugly and not informative}
    \label{fig:fk}
\end{figure}

==> fig/submethod.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/submethod.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
